Towards Adaptive Compliance

Mission critical software is often required to comply with multiple regulations, standards or policies. Recent paradigms, such as cloud computing, also require software to operate in heterogeneous, highly distributed, and changing environments. In these environments, compliance requirements can vary at runtime and traditional compliance management techniques, which are normally applied at design time, may no longer be sufficient. In this paper, we motivate the need for adaptive compliance by illustrating possible compliance concerns determined by runtime variability. We further motivate our work by means of a cloud computing scenario, and present two main contributions. First, we propose and justify a process to support adaptive compliance that ex- tends the traditional compliance management lifecycle with the activities of the Monitor-Analyse-Plan-Execute (MAPE) loop, and enacts adaptation through re-configuration. Second, we explore the literature on software compliance and classify existing work in terms of the activities and concerns of adaptive compliance. In this way, we determine how the literature can support our proposal and what are the open research challenges that need to be addressed in order to fully support adaptive compliance.

==> adaptive compliance arxiv/background.tex <==
\begin{figure}[t!!]
\centering
\includegraphics[scale=0.48]{figures/Dimensions.pdf} 
%\vspace{-5pt}
\caption{Compliance elements and dimensions.}
\label{fig:dimensions}
%\vspace{-15pt}
\end{figure}

\section{Compliance in Software}
\label{sec:background}

In the context of information systems, compliance refers to ``ensuring that an organisation's software and system conform with multiple laws, regulations and policies'' \cite{Zdun12IEEE}. From this definition we can distinguish two main elements in compliance: the \emph{system} and the \emph{compliance sources} that have to be conformed with. Moreover, the system runs in an \emph{operating environment}, that may affect the compliance sources against which the system has to conform. 
Figure~\ref{fig:dimensions} shows these elements and their different dimensions.
%The main compliance elements and their different dimensions are shown in Figure~\ref{fig:dimensions}. 

\footnotetext[2]{\url{http://www.hhs.gov/hipaa/}}
\footnotetext[3]{\url{https://www.congress.gov/bill/114th-congress/senate-bill/754}}

%Compliance sources are all the rules that can apply for a particular scenario. 
The \emph{type} of compliance sources refers to the kind of rules specified in the source. In particular, a compliance source can include regulations such as \hipaa\footnotemark[2], \cisa\footnotemark[3], and \gdpr\footnotemark[4]; standards such as \pci\footnotemark[5] and ISO/IEC 27000 series\footnotemark[6]; good practices; and internal policies within a particular organisation. \emph{Mandate} refers to the optional or mandatory character of the compliance source. For example, regulations are compulsory (e.g., \hipaa in the US) while standards and internal policies (e.g., ISO/IEC 27000 series) may not. The \emph{abstraction level} denotes the level of interpretation necessary to enact the statements mandated by a compliance source in a system. Regulations are usually expressed at a higher level of abstraction than standards and internal policies. For example, \gdpr requires companies to prove compliance without suggesting specific mechanisms, while an internal organisation policy may specifically state that rooted Android phones cannot connect to the company's internal network. Compliance sources apply to particular \emph{jurisdictions}, territories or spheres of activity. For example, \hipaa applies to US organisations dealing with personal healthcare information, while the \gdpr is intended to apply to any organisation delivering services to EU citizens. 





A system executes \emph{compliance controls}, which are implementations of the rules defined by a compliance source. For example, section 164.312(a)(2)(iii) within \hipaa mandates the implementation of procedures to log off from an electronic session after a predetermined time of inactivity. A compliance control to address this rule could involve forcing user sessions to expire after five minutes of inactivity. Compliance controls determine the \emph{compliance level} of a system with regards to its compliance sources. Three \emph{de-facto} levels of compliance are proposed in the literature \cite{colombo2014business}: `full compliance' when all rules are satisfied; `partial compliance' when all mandatory rules are satisfied; and `non-compliance' where one or more mandatory rules are not satisfied. 
 
% The operating environment is where the system runs, which may affect the compliance sources that apply and the compliance level of the system. 
Although the operating environment is highly dependent on the specific application domain, we distinguish two main characterising elements. First, the \emph{system users} who can reside and/or operate in different geographical locations and/or spheres of activity may need to comply with different compliance sources. Second, the \emph{physical or virtual infrastructure} where a system operates influences the applicable compliance sources and the compliance level that needs to be achieved. For example, IT systems in a US hospital have to comply with \hipaa and doctors who use personal devices to access patient records become part of the operating environment. 

\begin{figure}[t!!]
\centering
\includegraphics[scale=0.5]{figures/LifecycleAndArtifacts.pdf} 
%\vspace{-5pt}
\caption{Compliance management lifecycle.}
\label{fig:ComplianceArtefacts}
%\vspace{-15pt}
\end{figure}

\footnotetext[4]{\url{http://ec.europa.eu/justice/data-protection/}}
\footnotetext[5]{\url{https://www.pcisecuritystandards.org}}
%\footnotetext[5]{\url{https://www.pcisecuritystandards.org/documents/PCI_DSS_v3-1.pdf}}
\footnotetext[6]{\url{http://www.iso.org/iso/catalogue\_detail?csnumber=66435}}

\jesus{should we highlight the shortcomings of the existing lifecycle approaches?}

Different reference processes have been proposed in the literature to support compliance management ~\cite{cabanillas2011exploring, daniel2009business, ramezani2014supporting, Tilburg08}. Figure~\ref{fig:ComplianceArtefacts} presents a simplified compliance management lifecycle covering the main activities of these processes. Initially, \emph{compliance sources} are discovered depending on the system and its operating environment. Compliance sources are then interpreted to extract \emph{compliance requirements}, 
%an activity that is usually difficult and error-prone~\cite{otto2007addressing}. These requirements 
which are expressed as rules about actors and their rights and obligations on particular data objects~\cite{breaux2008analyzing}. 
%The interpretation of compliance sources can also help identifying overlaps and conflicts in compliance sources~\cite{gordon2011managing, ghanavati2014compliance}. 
During development, the requirements are implemented in the system as \emph{compliance controls}. 
Finally, compliance requirements and controls are evaluated to determine the compliance level they ensure and to assess how they can be improved, if necessary.





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> adaptive compliance arxiv/challenges.tex <==
%\vspace{-10pt}
\section{Research Challenges}
\label{sec:challenges}

Adaptive compliance poses a number of research challenges, some carried over from ``traditional'' compliance work, as well as some significant new ones. Open research challenges relevant to adaptive compliance but carried over from previous compliance research include:

\begin{inparaenum}[\itshape 1\upshape)]
\item \textbf{Compliance sources interpretation.} Multiple authors have proposed specific techniques to interpret regulations and extract compliance requirements, especially in requirements engineering. However, existing work is still limited, 
since this activity usually relies on the specific domain knowledge of the requirements engineers and is performed manually.

\item \textbf{Multi-jurisdictional requirements.} The analysis of overlaps between different regulations has also attracted attention, although existing approaches are only partially automated. In order to detect conflicts among different compliance sources at runtime, adaptive compliance requires more fully automated analysis than provided by current techniques. 

\item \textbf{Remedy for compliance violations.} Our work also highlighted the ongoing challenge of automated remedies for compliance violations. Although there are multiple proposals for automated compliance checking and diagnosis, existing mitigation techniques for violations usually require human intervention.
Since the adaptive compliance process has to handle violations at runtime, we need to provide the process with automated, dynamic mitigation approaches.
\end{inparaenum}

Our work also suggests that adaptive compliance raises new research challenges. We identify five main gaps in the literature that must be addressed:

\begin{inparaenum}[\itshape 1\upshape)]
\setcounter{enumi}{3}
\item \textbf{Compliance readiness.} 
We define compliance readiness as the capability of a system to foresee and comply with different compliance requirements. 
This capability requires awareness of different compliance sources and requirements that may apply to the system or its clients, and a pool of compliance controls, ready to be customised and invoked.
Although some authors have envisaged variability in business process rules to respond to variable compliance requirements, those approaches need to be extended for more complex controls and scenarios.


%% done?
\item \textbf{Compliance automation.} Currently, only compliance checking has been somewhat automated, and even so, 
often overlooking the impact of the operating environment.
Compliance sources discovery and interpretation remain to be automated, although there are some promising partial successes \cite{kerrigan2003logic, boella2013managing, toval2002legal}.
A repository of compliance sources and their different context dependent interpretations, could support this tedious and error-prone activity. Moreover, automating the reconfiguration  of compliance controls in order to correct compliance violations is needed.

%% done
\item \textbf{Runtime assurances.} Demonstrating compliance is often just as important as actually being compliant. There are several approaches to demonstrate compliance by tracing compliance requirements to regulations and compliance controls. However, existing support at runtime is more patchy, and focuses on compliance violations diagnosis, primarily considering systems but not their compliance sources nor their operating environment. Therefore, we need to extend the diagnosis to these elements, and provide evidence about if and how reconfigurations really increase compliance levels.

\item \textbf{Models for compliance controls and operating environment.} Our work shows multiple proposals to describe compliance rules and requirements, but very few to describe compliance controls and the operating environment. While the operating environment is highly dependent on the specific application domain, we think that a standard way to describe the compliance controls, their variability, and their impact on the system is necessary.

%% done
\item \textbf{Impact on performance.} Surprisingly, existing research has overlooked the effects of compliance on system performance. Since the adaptive compliance process is intended to handle compliance issues at runtime, performance is increasingly important. Therefore, more efficient ways are needed to check compliance, which has already been shown to be an NP-complete problem. Furthermore, empirical studies are needed to assess the impact on the system performance of executing compliance controls and monitoring the operating environment.
\end{inparaenum}






==> adaptive compliance arxiv/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

%% talk about related concepts like Partial Compliance and Compliance as a Service (CaaS)

In this paper, we have broadened the definition of com\-pliance-as-a-service scenario to motivate and encompass what we call adaptive compliance. We proposed a process to achieve adaptive compliance, and examined existing support for such a process in the software compliance literature. We found that most existing approaches focus on design time compliance, with little work addressing the increasing run-time variability found in compliance sources, systems, and their operational environment. We used the gaps we identified in the literature to suggest a number of research challenges to fully supporting adaptive compliance. Our primary aim in this paper was to raise awareness of these challenges, and to encourage the research community to address them. In our own future work, we plan to explore these challenges, focusing in particular on the issues of automation through runtime re-configuration.

%In this work, we have envisioned a Compliance-as-a-Service scenario to motivate the need of adaptive compliance. 
%We have also proposed a process to achieve adaptive compliance and to examine the existing support in the software compliance literature to it.
%As a result, we have discovered that most of the existing research approaches focus on design time, and consequently are insufficient to address runtime variability.
%The identified gaps in the literature have led to six research challenges that, together with ongoing challenges, must be tackled to fully support adaptive compliance.
%This is only the first step of a, we hope, long way. Our main intention with this work is to raise new concerns about software compliance, and to persuade different software research communities to test their solutions in this new scenario. In future works, we plan to explore several of those areas in an attempt to fulfil the adaptive compliance vision.


==> adaptive compliance arxiv/discussion.tex <==
%\vspace{-10pt}
\section{Conclusions and Future Work}
\label{sec:discussion}

In this paper, we have attempted to broaden the definition of compliance-as-a-service to include our idea for adaptive compliance. We have proposed a process to achieve adaptive compliance and discussed how existing work can support the various activities of our adaptive compliance process. A short review of the literature has identified that while existing approaches focus on design-time compliance, very little work has examined the increasing run-time variability found in compliance sources, systems and their operational environment. Furthermore, our review was used to identify several future research challenges which need to be addressed in order to fulfil our vision for adaptive compliance.

Although one of our main ambitions is to automate as much of the compliance process as is feasible, there are limits to this. 
Currently, we are better equipped to automate checking and enforcement of compliance rules.
However, neither all our proposed activities nor compliance rules can be fully automated. 
For example, a rule that specifies the behaviour of a security incident response team may need to be crafted manually, and its enforcement depends on enforcing human behaviour. 
This requires a discussion on the ``human-in-the-loop'' aspects of adaptive compliance. %about in which ways software can assist humans on compliance, and how these are involved in the process.

%For example, the extraction of compliance requirements and the implementation of compliance controls would require human intervention at least for the first time, even when using repositories for both.
%Furthermore, not all the compliance rules can be automatically performed. A rule that specifies the behaviour of a security incident response team may need to be crafted manually, and its enforcement depends on enforcing human behaviour. 

%Future research will examine several key areas that include a proper literature review, investigating how to automate the compliance process and examining the impact of adaptive compliance in other domains. 
Our future work will include conducting a more in-depth analysis of the literature to further investigate the compliance process gaps identified in this paper. The objective of this in-depth literature review would be to expand our understanding of related areas such as reconfiguration planning and execution in adaptive systems. As one of our main ambitions is to automate as much of the compliance process as possible, future work will need to examine which parts of the process can be automated and to what extent. This work will also look to address issues with automation through runtime re-configuration. Finally, future work will examine how our idea of adaptive compliance can be extended into other domains, such as the Internet of Things, where a myriad of heterogeneous and potentially untrusted devices interact. That could provide an additional and important cyber-physical perspective to adaptive compliance.

==> adaptive compliance arxiv/intro.tex <==
\section{Introduction}
\label{sec:intro}

% Software is the driving engine of modern society; most human
% activities, including critical ones, are either software-enabled or
% entirely managed by software. 
With software becoming increasingly pervasive, ensuring compliance to regulations, standards or policies is also becoming increasingly important to foster its wider adoption and acceptability by society and business. For example, in recent years, compliance with industrial regulations (e.g., \hipaa) and data security standards (e.g., \pci and ISO/IEC 27000-series) has become an essential requirement of some software systems. Non-compliance can result in loss of reputation, financial fines\footnote{\url{http://www.hhs.gov/about/news/2014/05/07/data-breach-results-48-million-hipaa-settlements.html}} or even criminal prosecution. 
%Consequently, achieving compliance has aroused the interest of both industry and academia ~\cite{Zdun12IEEE}.
Within acade\-mia, compliance has been examined in the areas of requirements engineering~\cite{otto2007addressing}, \soa~\cite{Tilburg08}, cloud computing~\cite{martens2011risk} and \bpm~\cite{fellman2014state}. 
Each of these has tackled compliance from different perspectives, including the interpretation of regulations into compliance requirements~\cite{breaux2008analyzing, ghanavati2014goal}, compliance checking~\cite{awad2008efficient, muller2014comprehensive}, and the definition of a reference process for compliance management~\cite{turetken2012capturing,martens2011risk}.

Ensuring compliance is more challenging in software systems that operate in heterogeneous, highly distri\-buted and changing environments, such as cloud computing services.
Cloud providers often deliver their services to clients from different geographical locations that have their own compliance requirements. Providing customised \emph{Compliance-as-a-Service} could relieve clients of the compliance burden and give providers a significant competitive advantage. However, cloud providers may still face different and multi-jurisdictional compliance requirements. They must also comply with the regulations that apply where their physical infrastructure resides. In a multi-tenancy environment, in which different clients may share computational resources, this could also lead to overlaps and conflicts between different compliance requirements. 
All this variability may in turn lead to compliance violations. Although compliance at runtime has gained attention recently \cite{birukou2010integrated, gomez2015compliance, ly2015compliance}, as far as we are aware, existing techniques are normally applied at design time and are unable to deal with this kind of runtime variability.

In this paper, we propose \emph{adaptive compliance} as \emph{the capability of a software system to continue to satisfy its compliance requirements, even when runtime variability occurs}. We motivate our work by using a \paas scenario and provide two main contributions. 
First, we propose and justify a process to support adaptive compliance that extends the traditional compliance management lifecycle with the activities of the Monitor-Analyse-Plan-Execute (MAPE) loop, and achieves adaptation through reconfiguration.
Second, we explore the literature on software compliance to identify which activities of our process are already supported and which present open research challenges. 
%To achieve this aim, we considered work published in the aforementioned software research areas.
Our ambition is to motivate the need of adaptive compliance and encourage researchers from the adaptive systems community to address these challenges.

The rest of the paper is organised as follows. Section~\ref{sec:background} introduces the main concepts and terminology adopted in software compliance. Section~\ref{sec:motivation} presents a motivating scenario that illustrates the concerns when handling runtime variability in compliance. Section~\ref{sec:solution} describes our adaptive compliance process and its existing support in the literature.  Section~\ref{sec:challenges} describes research challenges related to adaptive compliance. Finally, Section~\ref{sec:discussion} concludes the paper.





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> adaptive compliance arxiv/models.tex <==
\subsection{Models}
\label{sec:models}

Most of the research on compliance modelling has focused on compliance sources and requirements.
Multiple approaches have been proposed to represent regulations, using XML notations \cite{kerrigan2003logic}, UML  \cite{panesar2013supporting} or particular \dsls \cite{siena2013automated}.
Other works describe additional compliance sources, such \slas extending the WS-Agreement notation \cite{muller2014comprehensive}, or privacy policies using OWL-DL \cite{kahmer2008automating}. 
There are also numerous proposals to represent compliance requirements, especially by means of formal or semi-formal languages \cite{breaux2008analyzing, ghanavati2014goal, gordon2012reconciling} and \dsls \cite{birukou2010integrated, tran2012compliance}.
Nonetheless, the description of compliance controls and the operating environment appear to have been overlooked: while only few works on business processes address the former \cite{koetter2014integrating, SchummLMS10} by means of compliance descriptors and process fragments, the latter is even more neglected \cite{van2012context}, as we have presented in the previous sections.


%
%
%
%
%The MAPE loop requires models to describe all the potential sources of change \cite{Cheng2009}. In our case, these models should represent the different aspects of the system, the compliance sources and the operating environment.
%For the system, we have to describe the compliance controls and their configuration capabilities, but at the same time the configuration of the rest of the system, which might affect the compliance controls. 
%%In our \paas scenario for example, an update of the PostgreSQL database could have an impact on the cryptographic methods available for the data encryption compliance control.
%We also need to represent the compliance sources and their compliance requirements in a way that enact automated processing.
%Finally, the elements of the operating environment should be also described. Although the environment is highly dependent to the specific domain, we should consider at least, the virtual/physical infrastructure and the client needs. 
%
%\begin{table}[h!!]
%\centering
%\begin{tabular}{|p{1.8cm}|r|p{3cm}|}
%\hline
%\textbf{Element} & \textbf{Model} & \textbf{Proposals} \\
%\hline
%\multirow{2}{*}{\parbox{1.5cm}{\emph{Compliance} \\ \emph{sources}}} & Sources & \cite{kerrigan2003logic, kahmer2008automating, panesar2013supporting, siena2012capturing, muller2014comprehensive} \\
%\cline{2-3}
%& Requirements & \cite{gordon2011managing, ghanavati2014compliance, massey2010evaluating, brandic2010compliant, tran2012compliance, birukou2010integrated, awad2008efficient, reichert2012business, elgammal2014formalizing} \\
%\hline
%\multirow{2}{*}{\emph{System}} & Controls & \cellcolor{gray!30} \cite{koetter2013unifying, SchummLMS10} \\
%\cline{2-3}
%& System & \cite{panesar2013supporting}\\
%\hline
%\multirow{2}{*}{\parbox{1.5cm}{\emph{Operating} \\ \emph{environment}}}  & Infrastructure &  \cellcolor{gray!30}  \\
%\cline{2-2}
% & clients & \cellcolor{gray!30} \raisebox{1.5ex}[1.5ex]{\cite{van2012context}}\\
%\hline
%\end{tabular}
%\caption{Support for models on the literature.}
%\label{tab:models}
%\vspace{-5pt}
%\end{table}
%
%
%
%The description of regulations and standards has attracted the attention of several authors.
%\citet{kerrigan2003logic} propose an XML-based description of environmental regulations, decomposing the regulation text into a tree structure and adding First Order Predicate Logic statements.
%\citet{panesar2013supporting} also employ standardised notations, UML and OCL in this case, to describe conceptual models that provide succinct interpretations of safety standards, but also of the system.
%\citet{siena2012capturing} present a modelling framework and a specific language, Nomos2, to describe and analyse regulations and especially their variability in terms of different interpretations.
%
%There are other authors that focus on additional compliance sources, such as \slas, privacy policies or business process constraints. \citet{muller2014comprehensive} provide an extension of the WS-Agreement notation to describe \slas in \soa environments, while \citet{kahmer2008automating} provide a formal language, based on OWL-DL, and a tool, to define and compare privacy policies.
%On business processes, 
%\citet{awad2008efficient} employ a visual notation, BPM-Q, to describe process constraints. \citet{elgammal2014formalizing} also present a visual language, the so-named Compliance Request Language, which in this case is grounded on lineal temporal logic. The modelling approach of \citet{reichert2012business} relies as well on temporal logic, but without any particular extension.
%
%The description of compliance requirements has arisen considerable attention, especially in the requirements engineering community. \citet{massey2010evaluating} employ UML use cases to describe the compliance requirements with \hipaa of iTrust, an Electronic Health Records system. \citet{gordon2011managing} focus on multi-jurisdic\-tional requirements, and propose the semi-formalised Requirements Specification Language, employed to describe compliance requirements and find conflicts among different regulations. In the same line, \citet{ghanavati2014compliance} present the Legal-URN framework to describe regulatory requirements and find tradeoffs and prioritise between conflicting laws.
%\dsls have also gained traction to describe compliance requirements among authors in the \soa community. \citet{brandic2010compliant} propose their use to express compliance requirements in the cloud, while \citet{tran2012compliance} in particular present different \dsls to describe different types of compliance sources from different domains (e.g., security policies, regulations, or intellectual property licenses). \citet{birukou2010integrated}, in a similar way, employ specific \dsls to describe the compliance requirements for specific case studies, for example in the telecom domain.
%
%Nonetheless, the description of compliance controls or the operating environment has been overlooked on the compliance literature. 
%\citet{koetter2014integrating} propose to describe the configuration options of the compliance controls by means of the so-named compliance descriptors, by using an XML-based format.
%\citet{SchummLMS10} present process fragments to describe their compliance compliance controls, and natural text when fragments are not expressible enough.
%For expressing the operating environment, we only have found the work of \citet{van2012context}, who propose ontologies to describe the runtime context information. 
%
%The literature on software compliance presents many proposals to describe compliance sources and requirements, but very few for the rest of elements. This fact highlights the need to define models especially for the compliance controls and the operating environment, or bring them from other areas. 
%%The high number of works on the description of compliance sources and requirements points out the high received attention, but also means that it remains as an ongoing challenge. This is so especially for the case of describing rules and requirements from regulations, which are often abstract and complex to understand.
%
%
%
%


==> adaptive compliance arxiv/motivation.tex <==
\section{Motivating Scenario}
\label{sec:motivation}

In this section we present a \paas scenario, shown schematically in Figure~\ref{fig:PaaSScenario}, to motivate adaptive compliance and illustrate the main compliance concerns arising from runtime variability. The \paas provider offers customers a technological stack offering Database Management Systems (DBMS), run-time environments and various frameworks. The stack is deployed on top of an infrastructure which is hosted in the United States. Customers can deploy their own software applications using the stack offered by the \paas provider. 

The \paas provider also aims to provide \emph{compliance-as-a-service} to its clients, that is the capability to satisfy on-demand the compliance needs of its clients. As shown in Figure~\ref{fig:PaaSScenario}, initially the provider has to satisfy the compliance requirements of two different clients (Client 1 and 2). Client 1 operates in the US and stores patient health records, which are accessed by other third-party organisations. Hence, Client 1 has to comply with \hipaa regulations. Client 2 is also located in the US and handles its client's credit card information using the \paas. Therefore, Client 2 has to comply with \pci. Client 1 and Client 2 have differing compliance requirements, which the \paas provider must ensure are satisfied. 


% Existing research has traditionally addressed compliance from a static
% perspective focusing on the interpretation of compliance sources, the
% implementation of compliance controls and compliance checking. 

Although some cloud providers guarantee compliance for particular
regulations (e.g., HIPAA compliance by Catalyze\footnotemark[7]\footnotetext[7]{\url{https://catalyze.io/}} and
TrueVault\footnotemark[8]\footnotetext[8]{\url{https://www.truevault.com/}}), they are usually unprepared to satisfy emergent differing and varying compliance requirements. 
New \paas clients could introduce new compliance demands that need to be traded-off against those of existing clients who share the same execution platform. In our scenario, Client 3 is a new client providing financial services in the US and therefore requires a certifiable degree of privacy and security (e.g., ISO/IEC 27018). 
Clients can also change their compliance requirements due to changes in the jurisdictions that apply to their services. For example, Client 3 is considering expanding its operations to Europe and therefore it will need to comply with the European Union's \gdpr, which requires explicit user authorisation for any re-purposing of their personal data. This could result in a direct conflict with \cisa, which authorises sharing of personal data with federal institutions. 

Furthermore, variability in the compliance sources and the operating environment can also affect the compliance requirements and their satisfaction. 
In the case of compliance sources, Client 1, for example, could be required to comply with \cisa in the near future. 
While compliance sources may rarely evolve, changes in the system and its operating environment can occur more frequently. 
For example, updates to the DBMS may affect how data encryption is supported and hence, the satisfaction of the compliance requirements.
This also includes changes in the physical infrastructure of the service. 
In this sense, the \paas provider could move some of its data centres to Europe, which would trigger the need to comply with EU regulations for data retention and management.
The variability exposed by this scenario can be summarised by the following main concerns:
%With regards to the above scenario, we have identified four main concerns arising from runtime variability that need to be addressed:

\begin{figure}[t!]
\centering
\includegraphics[scale=0.42]{figures/PaaSScenario.pdf} 
\caption{PaaS Scenario.}
\label{fig:PaaSScenario}
%\vspace{-15pt}
\end{figure}

%
%Runtime variability brings four main concerns to be addressed to
%support adaptive compliance.

\begin{inparaenum}[\itshape a\upshape)]
\item \textbf{Awareness}. Runtime variability requires awareness of any changes that take place in the operating environment, the system and the compliance sources which can impact compliance satisfaction. In particular, \paas clients must be able to elicit and modify their preferences with respect to the compliance sources they need to satisfy. The provider also needs to be aware of infrastructure changes and assess how these changes impact the compliance requirements.

\item \textbf{Automation}: Compliance-as-a-service requires executing appropriate compliance controls using a dynamic approach. This would also involve automating the discovery and interpretation of compliance sources, as well as the identification and remedy of compliance violations and potential conflicts between compliance requirements. %Such conflicts can arise when different cloud clients share the same infrastructure need to comply with conflicting regulations.

\item \textbf{Assurance}: The service provider needs to produce assurances about whether or not the compliance level is that required by its clients. These assurances can be provided by collecting data, showing traceability between compliance controls and requirements or by delivering formal proofs.

\item \textbf{Performance}: The on-demand nature of cloud computing means that a cloud provider has to respond to changes in a timely manner so as to avoid service outages.
\end{inparaenum}

\jesus{connect these concerns with the next section}

%
%
%% Finally, the delivered capabilities should be reasonably efficient (e.g., the service delivery or the compliance checking), providing also assurances about how compliance is achieved.
%
%
%
%
%Only some of these concerns, such as compliance checking, have already been addressed in previous
%work. \citet{birukou2010integrated} discuss a runtime governance approach for
%compliance in \soa, focusing on design time and 
%runtime compliance checking.
%\citet{muller2014comprehensive} propose a runtime monitoring approach
%of quality of service and compliance properties for \soa; explanations
%related to the service level achieved are also provided.
%\citet{ly2015compliance} propose a framework to compare the different 
%runtime compliance checking approaches for business processes proposed in the
%literature. Among them, \citet{barnawi2015runtime} propose to
%customise  business processes in the cloud to enact self-monitoring of their compliance rules, 
%while \citet{gomez2015compliance} present a runtime compliance checking and
%diagnosis approach for \bpm based on constraint programming.
%However, as far as we are aware, existing work has mainly focused on
%runtime compliance checking only; and a more comprehensive approach for
%adaptive compliance covering
%the different concerns arising from runtime variability has yet to be developed.
%
%%In dynamic and highly-distributed scenarios, such as the presented \paas, the runtime variability is an additional issue for compliance.
%
%
%
%
%
%
%%\jesus{highlight how we could rely on a pool of compliance controls to comply with multiple regulations and standards. highlight also the overlaps and conflicts}
%
%%First, the clients may use the platform in an on-demand way, as usual in the cloud. This mean that the provider should be able to respond, also on-demand, to the compliance needs of the clients. For example, Client 2 needs to comply with \pci as much as they need the platform, so the provider must be ready to satisfy such need and have implemented the required compliance controls beforehand.
%%Second, different compliance sources may present overlaps or even conflicts when working together, as some authors have previously remarked \cite{gordon2012reconciling,Breaux2015RE}. For instance, the upcoming \cisa and \gdpr have opposed policies about collecting personal data for governmental agencies. This means that the provider cannot satisfy both of them at the same time, and might lead to a further issue if Client 1 (requires \cisa) and Client 3 (requires \gdpr) share the same platform infrastructure.
%%% what about the third one?
%
%
%%%% Local Variables: 
%%%% mode: latex
%%%% TeX-master: "paper"
%%%% End: 


==> adaptive compliance arxiv/problem.tex <==
\section{Runtime Variability in Compliance}
\label{sec:problem}

In dynamic and highly-distributed scenarios, such as the presented
\paas, the runtime variability is an additional issue for compliance.
Traditionally, compliance has been considered a static problem, where
the system has to meet particular compliance sources. These sources
evolve slowly (if they do), in terms of months or years, and so the
system does to stay compliant with them. Nonetheless, changes in the
operating environment occur much faster and oftener than in the system
or the compliance sources. This is so since software nowadays requires
multi-tenant, on-demand and customisation capabilities to meet client
needs, increasing then the degree of runtime variability.

Some authors have addressed particular issues of compliance at
runtime, but there is a lack of comprehensive support. In this sense,
compliance monitoring and checking are the two most popular issues
covered. \citet{ly2015compliance} and \citet{barnawi2015runtime}
specifically focus on the runtime monitoring of business processes,
proposing a framework to compare the different approaches in the
literature \cite{ly2015compliance} and particular techniques for
process monitoring in the cloud \cite{barnawi2015runtime}.
\citet{gomez2015compliance} present runtime compliance checking and
diagnosis for \bpm, while \citet{muller2014comprehensive} do the same
for \slas. \citet{birukou2010integrated} even talk about runtime
governance for compliance in \soa, although the main considered issues
are again monitoring and checking.
%\citet{koetter2013unifying} even talk about adaptation in the compliance management, and propose configurable compliance descriptors to link compliance requirements with their implementation as controls on the system.

\begin{figure*}[ht!!]
\centering
\includegraphics[scale=0.7]{figures/AdaptiveCompliance.pdf} 
\caption{Adaptive compliance process and activities.}
\label{fig:AdaptiveCompliance}
\end{figure*}

%\jesus{we have to define these four concerns and explain where they come from}
These scenarios present four main concerns to be addressed, i.e., variability, automation, assurances and performance, as presented for the \paas scenario.
\begin{itemize}
\item \emph{Variability}: the variability permeates the whole compliance process, from multiple compliances sources to meet to the runtime variability in the operating environment. 
%this is the main concern for runtime compliance, since changes in the operating environment may lead to compliance violations that must be addressed.

\item \emph{Automation}: compliance is a tedious process that demands to be automated as much as possible. 
% we should deal with the runtime variability in an automated way, so we do not require human intervention at runtime. %\jesus{I'm sure that automation is a concern, but not if this is the right description}

\item \emph{Assurances}: besides meeting the rules, compliance is also about proving that the system effectively complies.

\item \emph{Performance}: as usual at runtime, the system should be able to detect compliance issues and respond to them in a reasonably efficient way.
\end{itemize}
%\jesus{Complete this paragraph}

%% Variability
%% Automation
%% Assurance
%% Performance







%\jesus{connect the related work with the rest of the section}
%Compliance at runtime issues have been already considered in the literature. \citet{birukou2010integrated} propose a runtime compliance governance approach for Service Oriented Architectures, from modelling of compliance requirements to runtime monitoring of the current compliance state.
%\citet{ly2015compliance} and \citet{barnawi2015runtime} specifically focus on the runtime monitoring of business processes, proposing a framework to compare the different approaches in the literature \cite{ly2015compliance} and particular techniques for process monitoring in the cloud \cite{barnawi2015runtime}.
%\citet{koetter2013unifying} even talk about adaptation in the compliance management, and propose a configurable compliance descriptors to link compliance requirements with their implementation as controls on the system.
%\citet{boella2013managing} are concerned about the impact of changes in the system and regulations, and their impact on the compliance level. Although all these works highlight particular issues on runtime compliance, they adhere to such specific issues. On the contrary, in this paper we try to envision a comprehensive approach to deal with runtime variability in compliance.

%The changes in the operating environment occur much faster and oftener than in the system or the compliance sources. 
%For example, in the \paas scenario, new clients may appear and request the platform with different compliance needs, whose controls could conflict with existing clients.
%In the \byod scenario, new devices may appear at runtime, or the configuration or apps of the existing ones may change, which could potentially diminish the compliance level.
%Consequently, we need an approach to deal with this runtime variability in compliance, which should complement the existing traditional compliance approaches.

%\jesus{bring this to the problem section}
%As far as we are aware, most of the research on compliance regards the system, the compliance sources and the different stages and outputs of the compliance lifecycle. 
%However, the impact of the runtime variability has no received the required attention from the literature. Following, we describe two scenarios where this variability and its impact on compliance is evident.
%\jesus{I may need an example of how the runtime variability in the operating environments affects compliance.}



%The previously described scenarios also introduce the \emph{operating environment} as an extra element that affects compliance. We consider the operating environment as everything that affects the system and the compliance sources that apply, but it is not under direct control of the system. For instance, in the \paas scenario, the platform users, their compliance needs and the platform containers under their control are the operating environment.  
%In the case of the \byod scenario, the hospital employers and their devices make up the operating environment.

%\jesus{examples of particular changes/runtime variability that affect compliance}




%\jesus{intro and compliance scope of this paper}
%Although compliance involves organisations, companies, systems and more actors, in this paper we focus on and take the point of view of IT systems and their implementation of compliance. 
%In this section, we describe the particular compliance problem we address and its context. First, present an overview of compliance for IT systems, setting forth the main vocabulary and concepts. Second, we describe two particular scenarios, related to the cloud and \byod, where runtime variability affects compliance. Finally, we discuss in general terms the impact of runtime variability on compliance.



%\subsection{Compliance Overview}
%
%%\jesus{compliance introduction and meaning. compliance in SE. main elements (sources and system)}
%
%
%\subsection{Motivating Scenarios}
%
%In this section, we describe two highly dynamic and distributed scenarios, which poses additional challenges for compliance. In the first one, we present a \paas that has to respond to the compliance needs of different clients, while the second one is about a company implementing \byod while complying with \hipaa. Both scenarios help us motivate the problem of runtime variability in compliance, and the need of adaptive compliance as a solution.
%
%\subsubsection{PaaS Scenario}
%
%
%\subsubsection{BYOD Scenario}
%
%%\byod policies present multiple benefits but at the same time leads to new challenges, especially in security and privacy terms. 
%\byod refers to the employer policy of permitting employees to bring and use their personally owned devices (e.g. smartphones, laptop, tablets...) to access company resources. On the one hand, this practice is related to a productivity increase by the employees, while reducing required employer investment on employees equipment. On the other hand, \byod leads to serious privacy and security issues~\cite{miller2012byod}. 
%%% I have to reduce the second part of this paragraph
%From the employer's side, security is the main concern: the network could be infected because of malware from those devices (often untrusted), or sensitive data may end in user's devices, losing control of it. Before \byod, the devices were totally managed by the employer, which most the time ensured compliant by design. From the employee's side, however, the main issue is privacy: employers might want to have some degree of control or monitoring on employee's devices, which are also used for personal purposes. In this sense, the line between personal and employer data is blurred.
%
%\begin{figure}
%\includegraphics[scale=0.45]{figures/BYODScenario.pdf} 
%\caption{BYOD Scenario}
%\label{fig:BYODScenario}
%\end{figure}
%
%%% BYOD particular scenario
%In our particular \byod scenario, we present a hospital in the US that allows their employees to use their own devices. At the same time, the hospital is forced to comply with the \hipaa, and they are also willing to comply with the ISO standard on privacy (ISO/IEC 29100) \cite{iso29100}. 
%Due to \byod, many doctors in this hospital employ their own devices to check and register patient health's conditions. For example, Doctor1 employs his own iPad, while Doctor2 uses his Android tablet for this purpose (Figure~\ref{fig:BYODScenario}). The doctors employ these devices also for personal use, as usual in \byod, so they have installed different apps and have personal files in the devices. While the device of Doctor1 seems secure, the Doctor2's tablet allows to install apps from unknown sources and does not have an antivirus.
%
%Existing issues and threats of \byod get magnified when, for example, a hospital has to comply with \hipaa. 
%A stolen, lost or even compromised device may lead to protected health information leaks, and consequently to settlements and fines, something that has already happened \footnote{http://www.healthcarefinancenews.com/news/lahey-pays-850k-widespread-hipaa-non-compliance}. This means that if our doctors lose their personal devices, or get them infected by malware (likely to happen for Doctor2), the hospital might violate \hipaa compliance.
%Besides, the variability of devices and their configuration and installed apps in \byod pose an additional challenge for compliance. For example, our two doctors have two different devices (iPad and Android tablet), each one with different configuration, apps and their own threats, as shown in Figure~\ref{fig:BYODScenario}. 
%Although there are technologies to manage the connected devices (e.g, Mobile Device Management) remotely to configure them in the proper way for compliance, this might go against the privacy of the users. For example, analysing the outgoing traffic of the doctors devices to ensure compliance may invade their privacy.




%% particular policies
%% - support for blackberry, iOS and Android. particular configurations will be neccesary
%% - require the installation of a company app
%% - require the installation of particular antivirus
%% - devices should not be rooted or jailbroken
%% - devices should be updated to the newest available OS version
%% - healthcare data can only be accessed using containerization technology.

%% resources:
%% - internal network
%% - virtual machines & servers
%% - shared storage
%% - DB

%% technologies:
%% - Mobile-device Management (MDM) + NAC (Network Access Control)
%% - Containerization

%% issues and questions:
%% - maybe am I doing something that is already done?
%%   + the enabling technology already exists. 
%%   + which are the research challenges then?
%%   + RESEARCH CHALLENGE: How to be compliant with regulations and standards while allowing BYOD?
%% - where are the jurisdictions in this scenario? 
%%   + It could be the OS or type of device (Android, iOS, Windows...)
%% - what's the differente between adaptive security and adaptive compliance?
%%   + ??




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> adaptive compliance arxiv/relatedWork.tex <==
\section{Related Work}
\label{sec:related}

Compliance has attracted much attention from software engineering academics, especially in the areas of requirements engineering, \soa, cloud computing and \bpm. This has led several authors to survey the state of the art for general or particular purposes.
Most of the works in requirements engineering, as \citet{otto2007addressing} show, focus on interpreting the compliance sources and extracting, representing, analysing and reconciling compliance requirements. 
In the cloud area, \citet{martens2011risk} propose a reference model for risk and compliance management, based on a systematic literature review. However, the most prolific area for compliance is \bpm. In this sense, Tilburg University \cite{Tilburg08} present a literature review, in the context of an European project, focused on the discovery, specification and improvement aspects of compliance for services and business processes. \citet{fellman2014state} also survey the general state of the art cataloguing the literature in different dimensions, while \citet{el2012business} analyses the solutions proposed on regulatory compliance management. In this work we survey the literature in all these areas, but in our case to find out how good adaptive compliance can be supported with the existing research.

Compliance at runtime issues have been already considered in the literature. \citet{birukou2010integrated} propose a runtime compliance governance approach for Service Oriented Architectures, from modelling of compliance requirements to runtime monitoring of the current compliance state.
\citet{ly2015compliance} and \citet{barnawi2015runtime} specifically focus on the runtime monitoring of business processes, proposing a framework to compare the different approaches in the literature \cite{ly2015compliance} and particular techniques for process monitoring in the cloud \cite{barnawi2015runtime}.
\citet{koetter2013unifying} even talk about adaptation in the compliance management, and propose a configurable compliance descriptors to link compliance requirements with their implementation as controls on the system.
\citet{boella2013managing} are concerned about the impact of changes in the system and regulations, and their impact on the compliance level. Although all these works highlight particular issues on runtime compliance, they adhere to such specific issues. On the contrary, in this paper we try to envision a comprehensive approach to deal with runtime variability in compliance.

%% compliance governance and comprehensive approaches
Some other authors have proposed comprehensive compliance approaches to assist the compliance process during its whole lifecycle, especially for business processes. \citet{el2008towards} and \citet{ly2012enabling} discuss the requirements and challenges of frameworks for business process compliance management, and present their own approaches in this sense. In a similar line, \citet{cabanillas2011exploring} propose the concept of business process compliance management system, together with a lifecycle for compliance management and a set of challenges. \citet{ramezani2012separating} advocate for the separation of the compliance management from the business process, and also propose a lifecycle in this sense. \citet{tran2012compliance} propose a model-driven approach for compliance management in process-based SOA environments, with multiple views addressing different compliance concerns. \citet{daniel2009business} present a governance approach for SOA-based business processes, covering the whole lifecycle.



\jesus{should we include here and compare the compliance lifecycle proposals? We can discuss them here or in the compliance overview.}
%% lifecycle approaches:
%% - \citet{cabanillas2011exploring}
%% - \citet{ramezani2012separating}
%% - \citet{daniel2009business}
%% - \cite{Tilburg08}
%% - \citet{fellman2014state} %% for compliance checking




==> adaptive compliance arxiv/runtimeSolution.tex <==
\subsection{Monitor}

The literature on monitoring is mainly focused on system changes, neglecting the compliance sources and the operating environment. While compliance sources rarely change at runtime, the operating environment does, requiring a timely detection and response.
Several works have shown awareness of different monitoring factors, such as the system execution~\cite{birukou2010integrated}, the Quality of Service in \slas~\cite{muller2014comprehensive}, or time, resources and data in business processes~\cite{ly2015compliance}. However, the operating environment has only been considered for particular aspects of specific cases in the context of business processes~\cite{van2012context}.
Most of those works present approaches to automate the monitoring in business processes \cite{birukou2010integrated, van2012context} and \soa~\cite{muller2014comprehensive}.



 %Therefore, that is a lack which should be addressed. 


%The goal of monitoring, the initial runtime activity, is to identify changes that may affect the compliance level.
%The system must be aware of different sources of change and monitor them in an automated way.
%Changes in the operating environment and the system are likely to happen at runtime. 
%For example, new clients with different compliance needs may request the platform, whose updates in tech stack might also lead to changes in the available compliance controls.
%On the contrary, compliance sources evolve slowly, leading to discover new regulations o re-interpret the existing ones.
%The system has also be able to detect changes in a reasonable time and performance, and assure their provenance.
%In this sense, for example, we should be able to trace that the update of the database leaded to disable a particular encryption method.


%Monitoring changes that affect compliance have received some attention in the literature. However, we should be careful since several authors use ``compliance monitoring'' to refer both to runtime compliance monitoring and checking \cite{birukou2010integrated, ly2015compliance, barnawi2015runtime}. 
%\citet{muller2014comprehensive} propose an automated monitoring of the Quality of Service for \slas, gathering metrics such as response time or availability.
%On service-based business processes, \citet{birukou2010integrated} monitor the system execution and its events to detect potential compliance violations.
%Also for business processes, \citet{barnawi2015runtime} present a self-monitoring compliance approach for processes in the cloud, monitoring execution order and time in particular.
%\citet{ly2015compliance} go further and propose the monitoring not only of time, but also of resources and data at runtime for business processes.
%While the previous approaches focus on the system monitoring, \citet{van2012context} propose to automatically monitor context data (our operating environment.) by using ontologies to subsequently check compliance. 
%The work of \citet{boella2013managing} considers the evolution of the compliance sources, by extending the Eunomos legal knowledge management system. Nonetheless, the updates are not automated, and should be introduced by the software engineers in charge of the system.
%
%The existing monitoring approaches focus especially on the system \cite{muller2014comprehensive, barnawi2015runtime, birukou2010integrated, ly2015compliance}, while changes in the operating environment \cite{van2012context} or the compliance sources \cite{boella2013managing} have received less attention. 
%Some of these works consider different categories for the monitoring of the system, for instance \citet{ly2015compliance} consider time, resources and data, while \citet{van2012context} take into account specific elements in the context of the particular domain. 
%While most of the system monitoring approaches are automated, to the best of our knowledge there is no approach to automatically detect and track changes in the compliance sources.
%Furthermore, the existing proposals for monitoring seem to neglect assurances and performance concerns.


\subsection{Analyse}

Compliance analysis is the activity that most has attracted most attention from the research community, especially for checking compliance levels. 
However, additional awareness on the potential conflicts of multi-jurisdictional requirements \cite{ghanavati2014goal, gordon2012reconciling} or the impact of the operating environment \cite{Knuplesch15ER, van2012context} is necessary.
Compliance checking can take place at design time and at runtime. 
Design time checking approaches are common for business processes, and rely on a plethora of analytical techniques, such as those based on Petri Nets \cite{awad2008efficient, ramezani2012did} and temporal logic \cite{awad2008efficient, elgammal2014formalizing}. 
Similar approaches have been proposed for general regulatory compliance, by means of inference engines \cite{siena2013automated} and first order predicate calculus \cite{kerrigan2003logic}, and for business to business interactions \cite{molina2012model}.
Runtime compliance checking has gained momentum recently, especially in business processes \cite{birukou2010integrated, gomez2015compliance, van2012context} and \soa \cite{birukou2010integrated, muller2014comprehensive}.
Some of these compliance checking approaches also provide diagnosis support (i.e. assurances) for the causes of compliance violations \cite{gomez2015compliance, muller2014comprehensive, ramezani2012did}.
In general, checking automation and diagnosis are well covered at design and runtime. However, automated multi-jurisdictional analysis and the consideration of the operating environment for the checking remain as open challenges.
Moreover, the performance of all these approaches have been generally overlooked, although compliance checking has been proven to be np-complete for business processes \cite{colombo2014business}.



%% 1. check the interplay of the different compliance sources that apply. overlaps and conflicts
%% 2. check the compliance level.
%% 3. trace the compliance violations to their causes

%After detecting changes, we should analyse their impact on the compliance level.
%In the first place, we have to consider which compliance requirements apply to the new scenario. Requirements from different compliance sources may present overlaps or even conflicts that must be traded off (e.g., trying to meet \gdpr and \cisa at the same time in the \paas scenario). 
%In the second place, we must analyse the compliance level, a task better in the literature known as compliance checking. Compliance checking can be performed usually at three different times, i.e. design time, runtime or a posteriori, as several authors have identified \cite{el2008towards, ramezani2012did, reichert2012business, ly2015compliance}. This task may take into account only the system and the compliance sources, or additional aspects such as the operating environment.
%Finally, we also have to diagnose the cause of the detected compliance violations.
%In Table~\ref{tab:survey}, we consider the approaches that deal with requirements from multiple compliance sources or with aspects of the operating environment under the awareness concern.
%The different checking times are considered under the automation concern, while under the assurances and performance concerns we place compliance diagnosis approaches and works on compliance checking performance respectively.

%Design time compliance checking has attracted significant attention in the literature, especially in \bpm. 
%In this sense, we have to remark the work of \citet{colombo2014business}, who prove that the hardness of verifying compliance is NP-complete for partial compliance and coNP-complete for full compliance.
%About specific compliance checking proposals, \citet{awad2008efficient} present a checking approach for process constraints using Petri nets and temporal logic. 
%In a similar way, \citet{ramezani2012did} also employ Petri nets for compliance checking and compliance diagnosis when violations are detected, while \citet{elgammal2014formalizing} relies on temporal logic for the compliance checker they provide as part of their compliance management framework. 
%\citet{banescu2012measuring} focus on privacy compliance checking, quantifying the severity of the violations when personal data is repurposed.
%Apart from business processes, \citet{molina2012model} present a Contract Compliance Checker to check compliance in business to business interactions, describing the contract clauses using business rules. Focusing on regulatory compliance, \citet{siena2013automated} present the NRTool, which uses an inference engine to reason on regulations expressed on their Nomos2 language \cite{siena2012capturing}, while \citet{kerrigan2003logic} describe regulations in their own XML format and check their compliance using First Order Predicate Calculus.
%
%Runtime compliance checking has gained momentum recently, as shown by several literature reviews \cite{ly2015compliance, becker2012generalizability}. 
%\citet{birukou2010integrated} propose the definition of violation patterns to monitor compliance violations in \soa based business processes, while \citet{barnawi2015runtime} enable the self-monitoring of business process compliance in the cloud by defining patterns to adopt and configure their rules.
%\citet{van2012context} provide runtime compliance checking using the Semantic Web Rule Language and considering context data, which matches our operating environment.
%\citet{gomez2015compliance} present a framework not only for compliance checking in business processes but also for diagnosis using constraint programming, paradigm that is also employed by \citet{muller2014comprehensive}, who  check and diagnose compliance for \slas expressed in the WS-Agreement language.
%
%There are some other approaches of interest for the analysis, but no directly focused on compliance checking.
%\citet{Knuplesch15ER} measure how changes in organisations affect compliance when they have collaborative business processes. \jesus{this sounds like changes in the operating environment!}
%\citet{gordon2012reconciling} propose a framework to describe, identify and finally reconcile conflicting compliance requirements from different jurisdictions by means of a water marking method, while \citet{ghanavati2014goal} present a similar approach, based on the Legal-RUN framework, to identify not only conflicts but also regulation overlaps and suitable tradeoffs in such situations. The main drawback of both approaches is their lack of automation.
%\citet{hashmi2015normative} present an abstract formal framework to classify regulatory norms and provide formal semantics to compliance violations, in a similar way as \citet{ly2012enabling} describe formal compliance criteria for semantic constraints, state changes, process changes and healing compliance violations. 
%\jesus{this last sound interesting for the planning}
%
%
%
%\jesus{UPDATE THE TABLE!!!!}
%
%
%The compliance research community has devoted significant efforts for compliance checking, although there are still several gaps. In general, the checking automation is well covered at design \cite{awad2008efficient, ramezani2012did, elgammal2014formalizing, banescu2012measuring, molina2012model, siena2013automated, kerrigan2003logic} and runtime \cite{birukou2010integrated, barnawi2015runtime, van2012context, gomez2015compliance, muller2014comprehensive}, including several works that diagnose the causes of compliance violations \cite{muller2014comprehensive, ramezani2012did, gomez2015compliance}. However, the analysis of conflicting compliance requirements from multiple jurisdictions still needs automated support \cite{gordon2012reconciling, ghanavati2014goal}, as well as more approaches considering the operating environment for compliance checking \cite{van2012context, Knuplesch15ER} are required. Finally, and to the best of our knowledge, analysis performance issues have neglected in the literature, despite their proved high computational cost \cite{colombo2014business}.


%\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Survey on compliance checking %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item \cite{becker2012generalizability}
%%% this paper reviews the state of the art in model-based compliance checking for business processes.
%%% the authors propose a research roadmap for further research in compliance checking, highlighting that
%%% most of the compliance approaches only work for particular rules or cases
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% taxonomies on checking %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item \cite{el2008towards}
%%% this paper characterises different dimensions and types of compliance checking
%
%\item \cite{ramezani2012did}
%%% this work proposes compliance checking and diagnosis on business processes by means of petri nets.
%%% additionally, the authors identify diferent types of compliance checkings:
%%% - forward compliance checking -> enforce compliance
%%% - backward compliance checking -> detect and diagnose non-compliance
%
%\item \cite{reichert2012business}
%%% in this paper, the authors distinguish 3 types of compliance checking (a priori, runtime and a posteriori),
%%% provide two ways to define compliance rules, and discuss the impact of process changes in compliance
%
%\item \cite{colombo2014business}
%%% this work proves the hardness of regulatory compliance checking for business processes.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% checking approaches %%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item \cite{ramezani2012did}
%%% this work proposes compliance checking and diagnosis on business processes by means of petri nets.
%
%\item \cite{awad2008efficient}
%%% compliance checking on the order of the tasks in business processes (and in particular in BPMN notation)
%%% the authors also employ a visual notation to describe the rules
%
%\item \cite{ly2012enabling}
%%% this work preesents a static compliance checking at structural level for business processes.
%
%\item \cite{elgammal2014formalizing}
%%% this work proposes a Compliance Request Language, a visual pattern-based language, grounded on temporal logic, to describe compliance rules for business processes in order to be analysed later. The authors also present a software tool suite that implements the language and the verification
%
%\item \cite{van2012context}
%%% this paper considers contextual information at runtime for compliance checking in business processes
%%% the authors provide an implementation of their checking proposal using a framework for process mining
%
%\item \cite{kerrigan2003logic}
%%% this paper proposes first-order predicate calculus to check compliance with regulations, which are expressed in XML format
%
%\item \cite{banescu2012measuring}
%%% this paper proposes a privacy compliance checking technique for detecting privacy violations and measure their severity.
%
%\item \cite{siena2012capturing,siena2013automated}
%%% these works propose a description language for norms and situations and a tool (NRTool) to check compliance by means of an inference engine.
%
%%% SLA analysis
%
%\item \cite{muller2014comprehensive}
%%% this paper presents an approach to provide explanations (checking and diagnosis) for SLA violations at runtime
%
%\item \cite{molina2012model}
%%% this paper presents a compliance checking for B2B (business to business) interactions
%
%%%%%%%%%%%%%%%%%%%%%
%%% misc proposals %%
%%%%%%%%%%%%%%%%%%%%%
%
%\item \cite{birukou2010integrated}
%%% this work propose process compliance checking at runtime, after obtaining the data in the monitoring phase.
%%% however, this proposal is a framework, so the authors do not present any particular technique for the checking.
%
%\item \cite{koetter2014integrating}
%%% this work proposes the concept of compliance descriptor and explains how that concept can be used to ease compliance checking. for the checking implementation, they rely on existing approaches
%
%\item \cite{hashmi2015normative}
%%% this work presents an abstract approach for compliance checking in business processes, without relying on any particular formalism
%
%\item \cite{Knuplesch15ER} %% we could also use this work to motivate adaptive compliance
%%% this work focuses on the impact of business process changes for compliance. the authors propose the use of qualified dependency graphs to check which subset of the compliance rules might be affected because of the changes
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% multi-jurisdiction analysis %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item \cite{gordon2012reconciling,gordon2011managing} 
%
%\item \cite{ghanavati2014goal}
%\end{itemize}

\subsection{Plan}

To the best of our knowledge, the compliance literature presents very few works supporting the remedy of compliance violations. 
Although some authors have discussed the concept of compliance improvement \cite{ghose2007auditing, cabanillas2011exploring, ly2012enabling}, there is a lack of automated support. 
\citet{cabanillas2011exploring} state the need to provide recovery capabilities when compliance violations are detected at runtime.
\citet{ly2012enabling} discuss the notion of healable compliance violations, i.e. violations that can be fixed by restructuring the process or inserting additional branches, while \citet{ghose2007auditing} present a partially automated technique, based on structural and semantic patterns, to modify non-compliant processes in order to restore compliance. 
Our vision to enact compliance improvement is through the reconfiguration of the compliance controls. In this sense, several authors have proposed configuration capabilities for implementing compliance, as shown in Section~\ref{subsec:Implement}. However, none of these present specific techniques to remedy violations when detected.


%% our main contribution relies here: the configuration

%If we detect compliance violations in the previous activity, we have to reconfigure the compliance controls to improve the compliance level. For example, this could consist of setting the max number of failed login attempts to three. However, we may not achieve a full compliance in cases where different compliance requirements conflict, as in the case of personal data sharing for \gdpr and \cisa. That could lead to partially-compliant reconfigurations.
%In this activity, the awareness concern refers to the different available options (reconfigurations in our case) to improve the compliance level, the automation concern is about automating the analysis of such options to select the best one, the assurances is about proving how the result enhances compliance, and the performance is about the activity execution time.

%Some authors have discussed compliance restore at design time. For example, \citet{ly2012enabling} discuss the notion of healable compliance violations, i.e. violations that can be fixed restructuring the process or inserting additional branches, while \citet{ghose2007auditing} present a partially automated technique, based on structural and semantic patterns, to modify non-compliant processes in order to restore compliance. 
%At runtime, \citet{cabanillas2011exploring} state the need to provide recovery capabilities when compliance violations are detected. They propose a compliance-aware business process lifecycle, and identify the configuration and the compliance enactment as an activities of such lifecycle, but without specific techniques.
%Other authors have considered the concept of configuration for compliance, but without applying it for runtime compliance improvement. These are the cases of \citet{koetter2013unifying}, who consider consider configuration options for the compliance controls, which are described in their compliance descriptors;  \citet{schleicher2009maintaining}, who describe configuration options in business processes using variability descriptors; and \citet{ramezani2014supporting}, who present configurable rules for business processes.
%
%\jesus{UPDATE the table!!}
%
%To the best of our knowledge, runtime compliance improvement has been neglected in the literature. Although some authors have discussed the concept of compliance improvement \citet{ghose2007auditing, cabanillas2011exploring, ly2012enabling}, even at runtime \cite{cabanillas2011exploring}, there is a lack of fully automated approaches. 
%Our vision to enact compliance improvement is through the reconfiguration of the compliance controls, and in this sense, several authors have proposed configuration capabilities for compliance. However, none of them apply them for the improvement.
%In this sense, we are aware about are other areas in the literature that may be worth to explore for this activity, such as adaptive systems.



\subsection{Execute}

%Finally, we have to execute the previously defined reconfiguration of the compliance controls. The result of this activity should be a new running configuration that increases the compliance level.

The literature has not paid attention to this activity beyond works on configuration capabilities for compliance.
In our view, the key concerns of this activity should be the automated execution, in a timely manner, of reconfigurations that improve the compliance level. Assurances about how the reconfiguration execution has improved the compliance level should also be provided.





==> adaptive compliance arxiv/solution.tex <==
\begin{figure*}[ht!!]
\centering
\includegraphics[scale=0.7]{figures/AdaptiveComplianceProcess.pdf} 
\caption{Adaptive compliance process.}
\label{fig:AdaptiveCompliance}
\vspace{-10pt}
\end{figure*}



\section{Adaptive Compliance}
\label{sec:solution}

\jesus{read the beginning of this section again}

\jesus{discuss the differences with the traditional MAPE loop and the limitations (human-in-the-loop?)}

In this section we present a process to achieve adaptive compliance and a summary of the support provided by the existing literature. This process, shown in Figure~\ref{fig:AdaptiveCompliance}, extends the compliance management lifecycle of Figure~\ref{fig:ComplianceArtefacts} with added support for variability runtime concerns through the MAPE loop. %~\cite{Kephart03Autonomic}. 
The adaptive compliance process begins with the automated \emph{discovery} of compliance sources with which the system needs to comply. Factors that influence the discovery of compliance sources include the system's physical location, its sphere of activity and the potential stakeholders. 
Next, the compliance sources must be \emph{interpreted} in order to identify the compliance requirements, which demand close collaboration between legal and domain experts, and software engineers~\cite{otto2007addressing}.
This activity could benefit from mechanisms to share and reuse compliance requirements, such as a multi-organisation repository. 
The requirements are subsequently \emph{implemented} in the system as compliance controls. Since the system is intended to meet differing compliance needs at runtime, the compliance controls should be flexible enough to be enabled, disabled and customised when required. 

At runtime, the system must \emph{monitor} its own state, the operating environment and the compliance sources. Any changes in these elements may result in either compliance violations or a reduced compliance level. While changes in compliance sources take place slowly, changes in the system or the operating environment often require a response at runtime. %% talk about probes for monitoring
When changes are detected, the system must \emph{analyse} their impact on the compliance level. First, overlaps  between the applying compliance requirements should be analysed, since they might lead to conflicts and consequently compliance violations. Second, the compliance level must be checked and if compliance violations are found, these must be diagnosed to determine their causes. 
In that case, the system needs to \emph{plan} a reconfiguration of the compliance controls to improve the compliance level when possible. 
Finally, the computed reconfiguration must be \emph{executed} in the system, effectively improving the compliance level.

This process requires of ``live'' models, especially at runtime to enact the Knowledge (K) component of the MAPE loop. 
Such models must describe the compliance sources and its requirements, the system and its compliance controls, and also the operating environment, including user preferences and the system infrastructure. 
The relevance of these models depends on the particular activities.
Some of them are more important at design time (e.g., compliance sources for their discovery and interpretation), while others are necessary at runtime (e.g., operating environment for the monitoring, or compliance controls for the plan). %% we should further discuss this in the future


%\jesus{motivate how the process addresses the concerns?}
In the following, we explore how the compliance literature supports the adaptive compliance activities and addresses the concerns presented in Section~\ref{sec:motivation}. This analysis allows us to identify topics which have been well discussed, along with gaps leading to research challenges. Table~\ref{tab:survey} relates existing approaches supporting the activities with the concerns that these approaches have addressed. Partially addressed areas are shown in light grey, while areas not addressed are shown in dark grey. %Row ``others'' covers additional concerns that are not immediately relevant to adaptive compliance.



\begin{table*}[ht!!]
\centering
\begin{tabular}{|l r|p{1.6cm}|p{1.6cm}|p{1.8cm}|p{1.7cm}|p{1.8cm}|p{1.6cm}|p{1.6cm}|}
%\cline{3-9}
%\thickcline{3-9}
\cline{3-9}
\multicolumn{2}{c}{} & \multicolumn{7}{|c|}{\textbf{Adaptive Compliance Activities}} \\
\cline{3-9}
\multicolumn{1}{c}{} & & \multicolumn{1}{c|}{\textbf{Discover}} & \multicolumn{1}{c|}{\textbf{Interpret}} & \multicolumn{1}{c|}{\textbf{Implement}} & \multicolumn{1}{c|}{\textbf{Monitor}} & \multicolumn{1}{c|}{\textbf{Analyse}} & \multicolumn{1}{c|}{\textbf{Plan}} & \multicolumn{1}{c|}{\textbf{Execute}} \\
\hline
\multirow{5}{*}[-6ex]{\rotatebox{90}{\textbf{Concerns}}}
& \multicolumn{1}{|r|}{ \textbf{Awareness}} & \cellcolor{gray!30} \cite{kerrigan2003logic,otto2007addressing,Tilburg08} & \cite{boella2013managing, breaux2008analyzing, Ghanavati:2015:ILI:2821464.2821473, ghanavati2014goal, gordon2012reconciling, maxwell2012managing, schmidt2012assessing, siena2013automated} & \cellcolor{gray!30} \cite{koetter2014integrating, ramezani2014supporting, schleicher2009maintaining} & \cellcolor{gray!30}
\cite{birukou2010integrated, ly2015compliance, muller2014comprehensive, van2012context} & \cellcolor{gray!30}
\cite{ghanavati2014goal, gordon2012reconciling, Knuplesch15ER, van2012context}
 & \cellcolor{gray!30} \cite{cabanillas2011exploring, ghose2007auditing, ly2012enabling} & N/A \\
\hhline{|~ |-|-|-|-|-|-|-|-|} 
& \multicolumn{1}{|r|}{\textbf{Automation}} & \cellcolor{gray!30}
\cite{boella2013managing,kerrigan2003logic}&
\cellcolor{gray!30} \cite{panesar2013supporting, toval2002legal, tran2012compliance, turetken2012capturing} &  \cellcolor{gray!30} \cite{ramezani2014supporting, SchummLMS10, tran2012compliance} & \cite{birukou2010integrated, muller2014comprehensive, van2012context} & \cite{awad2008efficient, birukou2010integrated, elgammal2014formalizing, gomez2015compliance, kerrigan2003logic, molina2012model, muller2014comprehensive, ramezani2012did, siena2013automated, van2012context} & \cellcolor{gray!100} \cite{ghose2007auditing} & \cellcolor{gray!100} \\
\hhline{|~ |-|-|-|-|-|-|-|-|} 
& \multicolumn{1}{|r|}{\textbf{Assurances}} & N/A &
\cite{boella2013managing, breaux2008analyzing, Ghanavati:2015:ILI:2821464.2821473, siena2013automated, turetken2012capturing}
& \cite{panesar2013supporting, tran2012compliance} & N/A & \cite{gomez2015compliance, muller2014comprehensive, ramezani2012did} & \cellcolor{gray!100} & \cellcolor{gray!100} \\ 
\hhline{|~ |-|-|-|-|-|-|-|-|} 
& \multicolumn{1}{|r|}{\textbf{Performance}} & N/A & N/A & \cellcolor{gray!100} & N/A & \cellcolor{gray!100} \cite{colombo2014business} & \cellcolor{gray!100} & \cellcolor{gray!100} \\
\hhline{|- |-|-|-|-|-|-|-|-|} 
\end{tabular}
\caption{Overview of the literature, structured by the concerns and activities of adaptive compliance.}
\label{tab:survey}
\vspace{-10pt}
\end{table*}



\subsection{Discover}

\jesus{what do we mean with each concern? -> awareness and automation}
Although discovery is a fundamental activity in the compliance management lifecycle, it has received little attention from the research community. 
Some studies have highlighted its importance~\cite{otto2007addressing, Tilburg08}, but without defining factors that affect applying compliance sources. % or any other specific approach.
Some studies have provided repository tools \cite{boella2013managing, kerrigan2003logic}. \citet{kerrigan2003logic} describe environmental regulations by means of an XML-based format and facilitate the discovery through searchable concept hierarchies. \citet{boella2013managing} provide the Eunomos web-based system to manage knowledge about laws and legal concepts in the financial sector.
However, in general, discovery lacks automated support and a general taxonomy of factors.



%\jesus{how existing work can help on that}
%Although discovery is a fundamental activity in the
%compliance management lifecycle~\cite{Tilburg08,otto2007addressing},
%it has not gained much attention from the research community. 
%\citet{otto2007addressing} highlight the need to discover in advance relevant
%laws and regulations that can constrain the application of a specific
%compliance source. However, they do not identify specific factors that
%can affect the discovery. To support automated discovery of relevant compliance
%sources \citet{kerrigan2003logic} present an XML-based repository for
%representing federal and state regulations and a document repository.
%This framework facilitates the discovery of specific regulations
%through searchable concept hierarchies. More recently,
%\citet{boella2013managing} proposed Eunomos, a
%web-based system to manage knowledge about laws and legal concepts in
%the financial sector. This tool can be used to search, classify and
%annotate legal knowledge, and to map the rules obtained from the
%knowledge to business processes. 

% Some authors have identified the discovery as a key a \cite{Tilburg08,otto2007addressing} for compliance management, but without any further proposal. In this sense, surveys the literature, only finding a few tangential works. 
% They aim to  environmental compliance sources with additional compliance checking capabilities.

%However, existing proposals focus on particular legislation documents
%(e.g., environmental policies, financial regulations) and are not general
%enough to identify compliance sources depending
%on the physical location and the sphere of activity of a system and
%its operating environment. It is therefore necessary to offer more
%comprehensive repositories covering a wider spectrum of laws, regulations,
%and policies. These repositories must provide enhanced searching
%functionalities based on the different factors brought by the system and its
%operating environment.
%\jesus{I see a lack of support in this sense. This leads to a research challenge}


\subsection{Interpret}

The interpretation of compliance sources has been widely covered by the research literature~\cite{otto2007addressing}.
However, most of the existing work relies on partially or totally manual techniques to extract compliance requirements. 
These techniques include Semantic Parameterisation~\cite{breaux2008analyzing}, goal based analysis, and CPR (commitment, privilege and right) analysis~\cite{schmidt2012assessing}, which have been validated by means of empirical studies.
Some authors have focused on compliance requirements variability, and in particular on the multiple possible interpretations of a regulation~\cite{boella2013managing, Ghanavati:2015:ILI:2821464.2821473, siena2013automated} and the evolution of the requirements~\cite{maxwell2012managing}. %% me cargo alguno mas?
The analysis and reconciliation of potentially conflicting mul\-ti-jurisdictional requirements have also received attention~\cite{gordon2012reconciling, ghanavati2014goal}.
In terms of automation, some research efforts have focused on the description of compliance requirements by using different approaches, such as \dsls \cite{tran2012compliance}, UML \cite{panesar2013supporting} or semi-formal representations \cite{turetken2012capturing}. A repository of compliance requirements has also been proposed~\cite{toval2002legal}, although without real tool support.
Assurances demonstrating the correctness of compliance requirements with respect to the sources have been suggested, especially in terms of traceability links \cite{breaux2008analyzing, Ghanavati:2015:ILI:2821464.2821473}  and formal proofs \cite{turetken2012capturing, boella2013managing, siena2013automated}.

%Extracting compliance requirements from legal texts or standards is a
%difficult and error-prone activity~\cite{otto2007addressing} due to
%the legal and domain-specific terminology employed. Interpretation of
%compliance sources thus requires close collaboration between legal and
%domain experts and software engineers~\cite{Zdun12IEEE}. The interpretation of compliance sources has been widely covered by
%the research literature~\cite{otto2007addressing}. For example, 

%Breaux et al. \cite{breaux2008analyzing} apply Semantic Parameterisation to regulation texts by rephrasing rights and
%obligations into restricted natural language statements (RNLS). 
%Identified constraints -- corresponding to specific actions (e.g.,
%disclosures or uses) or modalities (e.g., rights or refrainments) -- are
%recorded into a rule table. The authors solve ambiguities by maintaining
%cross-references between extracted constraints and the legal text, and
%also by introducing domain knowledge
%that is missing in the regulation~\cite{breaux2008legal}. Empirical
%studies have also been conducted (e.g.,~\cite{schmidt2012assessing}) to 
%measure the ability of requirements engineers to extract
%compliance requirements from policy documents. For example, \citet{schmidt2012assessing} reveal that  the requirements extracted
%by using CPR (commitment, privilege, and right) analysis lead to a
%higher percentage of identified compliance requirements, while the
%adoption of a goal based analysis produced requirements that could 
%have not been inferred directly from the policy. 
%
%The description of compliance requirements using \dsls or formal
%representations has also received attention~\cite{otto2007addressing}.
%For example, \citet{brandic2010compliant} propose the use of \dsls to
%describe compliance requirements, while
%\citet{panesar2013supporting} propose UML and OCL to describe and link
%the application  domain and the compliance
%sources.~\citet{tran2012compliance} propose a set of \dsls to
%represent concepts and rules of different compliance domains (e.g.,
%security, jurisdictional, intellectual properties). \citet{turetken2012capturing} provide control pattern templates to
%help compliance and business experts specify structured and
%semi-formal representations of recurrent types of controls for
%business processes. Such controls can affect the order of
%activities of a business process, authorisations on resources,
%segregation of duties, and temporal rules over process
%activities. Identified control patterns can be translated automatically into formal rules that are used for subsequent
%compliance assurance activities. 
%
%
%Variability awareness
%is very important for the interpretation activity as extracted compliance requirements can have
%multiple possible interpretations~\cite{graydon2012arguing}, can
%potentially evolve in the future~\cite{maxwell2012managing}, and can
%overlap and even conflict~\cite{gordon2011managing} -- in the case of
%multiple applying regulations. For example, regulations and standards
%as \hipaa or \pci have been interpreted in different ways and have
%also evolved over time. In particular, \hipaa had multiple amendments
%since 1996, while \pci has evolved through several versions (the
%current one is 3.1). In this sense, Gordon et
%al.~\cite{gordon2012reconciling,gordon2011managing} address
%multi-jurisdictional compliance requirements, first detecting overlaps
%and potential conflicts among different compliance
%sources~\cite{gordon2011managing} and then proposing techniques to
%reconcile them~\cite{gordon2012reconciling}. Similarly,
%\citet{ghanavati2014goal} propose a modelling framework (Legal-URN)
%to comply with multiple regulations, identifying different cases when
%two regulations can overlap. The Eunomos knowledge representation
%system~\cite{boella2013managing} has also been enhanced to deal
%with conflicts and overlaps among different
%regulations~\cite{ghanavati2014compliance} and to handle
%variability arising from multiple
%interpretations~\cite{Ghanavati:2015:ILI:2821464.2821473}.
%\citet{siena2012capturing} developed a modelling framework to express
%variability in regulations and  identify
%possible ways in which such regulations can be satisfied. Legal knowledge is expressed as clauses
%containing antecedents and consequents; compliance is
%evaluated through the applicability and satisfiability of these
%clauses for given sets of requirements.
%Finally, \citet{maxwell2012managing} propose
%an adaptability framework to identify the parts of a regulation that
%are more prone to change.
%
%Assurances demonstrating that
%compliance requirements express compliance sources correctly should
%also be provided. The most common ways to do so are by establishing traceability links from
%requirements to legal
%text~\cite{breaux2008analyzing,massey2010evaluating,Ghanavati:2015:ILI:2821464.2821473},
%or by formally proving that the requirements satisfy a set of
%regulations modelled formally~\cite{turetken2012capturing,boella2013managing,siena2012capturing}.
%
%
%
%
%
%
%
%
%
%%\jesus{the description of the reqs could be interesting for the Knowledge component of the MAPE loop.}
%
%
%Although the
%interpretation activity itself cannot be automated, extracted
%compliance requirements should be shared and re-used among
%practitioners and researchers. In this respect there is a lack of
%knowledge reuse mainly because this could lead some organisations to
%lose their competitive advantage or may raise confidentiality issues.
%Initiatives providing shared repositories of compliance
%requirements~\cite{toval2002legal} have only been proposed in the academia
%and more support, especially from the industry, is required.




\subsection{Implement}
\label{subsec:Implement}


Compliance implementation has received attention and partial automated support, in particular from the \bpm community.
Several works have considered configurable compliance controls for business processes, in the form of compliance descriptors~\cite{koetter2014integrating}, business process templates~\cite{schleicher2009maintaining} and configurable compliance rules~\cite{ramezani2014supporting}.
Implementation automation has been addressed from different perspectives. While some approaches have proposed an automated derivation of compliance controls from the requirement descriptions~\cite{tran2012compliance}, others have presented repositories of reusable process fragments~\cite{SchummLMS10} or compliance rules~\cite{ramezani2014supporting}.
Some of these also provide support for implementation assurances by explicitly linking compliance controls and requirements~\cite{tran2012compliance}, and concepts of the compliance source to the application domain~\cite{panesar2013supporting}.
However, the impact of compliance controls on the system performance has been surprisingly neglected. 







% Once we have identified the compliance requirements, we implement them

%Implementation of compliance controls should be flexible enough to
%incorporate variability awareness in compliance requirements. This relates to
%the capability of a software system  to be \emph{compliant-ready}, i.e.
%being able to enable, disable, or configure different compliance controls flexibly at
%different execution points in a short time. For example, limitation in
%the maximum number of login attempts and data encryption
%are compliance requirements mandated by existing regulations (e.g., HIPAA) and
%standards (e.g., PCI-DSS or ISO27000). They could be implemented by reusing
%the same compliance control modules, which can be enabled
%at specific execution points. Their particular configurations (e.g., time interval, max number of login attempts, or specific
%encryption techniques) should be determined depending on
%the particular compliance source and its interpretation.


% In the \bpm area, existing
%work has addressed variability awareness issues. For example, \citet{koetter2013unifying} propose the notion of
%compliance descriptors to link compliance requirements to compliance
%controls. Compliance descriptors are subsequently applied to
%implement compliance rules in business
%processes~\cite{koetter2014integrating}. Similarly, \citet{ramezani2014supporting} propose configurable
%compliance rules for business processes and provide a repository of
%them. Rules applying to the business process can be selected and
%configured using
%question trees. \citet{schleicher2009maintaining} employ the concept
%of business process template, which contains compliance constraints
%and points of variability, to ensure compliance in configurable
%business processes. Although other work has tackled compliance
%implementation, it does not focuses explicitly on variability and compliance controls configuration. For example,
%\citet{SchummLMS10} propose the use (and reuse) of process fragments
%to achieve compliance in business processes. In the \soa area,
%\citet{tran2012compliance} automatically derive compliance controls from the
%description of compliance requirements by using their proposed
%DSLs. 
%
%The aforementioned approaches have addressed automation issues in compliance
%implementation by fostering the generation, sharing and re-use of compliance
%controls, mainly for business processes.  However, applicability to a
%wider set of systems, such as cloud-based and pervasive applications
%is required. Moreover, more automation is required for the identification of the execution points in which
%compliance controls should be enabled and to support their configuration.
%
%Other work~\cite{brandic2010compliant,faniyi2012self} has particularly focused on assurance concerns, such as
%providing guarantees of certifiable and auditable compliance levels.
%For example, \citet{brandic2010compliant} propose a framework for specifying compliance requirements
%concerning security, privacy, and trust by leveraging compliance level
%agreements. They also propose a 
%middleware responsible for the deployment of certifiable
%and auditable applications, for provider selection in
%compliance with the user requirements, and for enactment
%and enforcement of compliance level agreements. \citet{faniyi2012self}
%present a resource control mechanism based on market control theory
%and reputation metrics to automate and adapt resource allocation in
%order to achieve \sla compliance.
%
%
%To our knowledge, performance issues in compliance implementation have
%been minimally covered by the research literature. Overheads
%determined by the execution of compliance controls, as well as any negative
%impact on the satisfaction of other software qualities, should be taken
%into account when compliance controls are implemented.






%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

%% talk about related concepts like Partial Compliance and Compliance as a Service (CaaS)

In this paper, we have broadened the definition of com\-pliance-as-a-service scenario to motivate and encompass what we call adaptive compliance. We proposed a process to achieve adaptive compliance, and examined existing support for such a process in the software compliance literature. We found that most existing approaches focus on design time compliance, with little work addressing the increasing run-time variability found in compliance sources, systems, and their operational environment. We used the gaps we identified in the literature to suggest a number of research challenges to fully supporting adaptive compliance. Our primary aim in this paper was to raise awareness of these challenges, and to encourage the research community to address them. In our own future work, we plan to explore these challenges, focusing in particular on the issues of automation through runtime re-configuration.

%In this work, we have envisioned a Compliance-as-a-Service scenario to motivate the need of adaptive compliance. 
%We have also proposed a process to achieve adaptive compliance and to examine the existing support in the software compliance literature to it.
%As a result, we have discovered that most of the existing research approaches focus on design time, and consequently are insufficient to address runtime variability.
%The identified gaps in the literature have led to six research challenges that, together with ongoing challenges, must be tackled to fully support adaptive compliance.
%This is only the first step of a, we hope, long way. Our main intention with this work is to raise new concerns about software compliance, and to persuade different software research communities to test their solutions in this new scenario. In future works, we plan to explore several of those areas in an attempt to fulfil the adaptive compliance vision.


==> problem.tex <==
\section{Runtime Variability in Compliance}
\label{sec:problem}

In dynamic and highly-distributed scenarios, such as the presented
\paas, the runtime variability is an additional issue for compliance.
Traditionally, compliance has been considered a static problem, where
the system has to meet particular compliance sources. These sources
evolve slowly (if they do), in terms of months or years, and so the
system does to stay compliant with them. Nonetheless, changes in the
operating environment occur much faster and oftener than in the system
or the compliance sources. This is so since software nowadays requires
multi-tenant, on-demand and customisation capabilities to meet client
needs, increasing then the degree of runtime variability.

Some authors have addressed particular issues of compliance at
runtime, but there is a lack of comprehensive support. In this sense,
compliance monitoring and checking are the two most popular issues
covered. \citet{ly2015compliance} and \citet{barnawi2015runtime}
specifically focus on the runtime monitoring of business processes,
proposing a framework to compare the different approaches in the
literature \cite{ly2015compliance} and particular techniques for
process monitoring in the cloud \cite{barnawi2015runtime}.
\citet{gomez2015compliance} present runtime compliance checking and
diagnosis for \bpm, while \citet{muller2014comprehensive} do the same
for \slas. \citet{birukou2010integrated} even talk about runtime
governance for compliance in \soa, although the main considered issues
are again monitoring and checking.
%\citet{koetter2013unifying} even talk about adaptation in the compliance management, and propose configurable compliance descriptors to link compliance requirements with their implementation as controls on the system.

\begin{figure*}[ht!!]
\centering
\includegraphics[scale=0.7]{figures/AdaptiveCompliance.pdf} 
\caption{Adaptive compliance process and activities.}
\label{fig:AdaptiveCompliance}
\end{figure*}

%\jesus{we have to define these four concerns and explain where they come from}
These scenarios present four main concerns to be addressed, i.e., variability, automation, assurances and performance, as presented for the \paas scenario.
\begin{itemize}
\item \emph{Variability}: the variability permeates the whole compliance process, from multiple compliances sources to meet to the runtime variability in the operating environment. 
%this is the main concern for runtime compliance, since changes in the operating environment may lead to compliance violations that must be addressed.

\item \emph{Automation}: compliance is a tedious process that demands to be automated as much as possible. 
% we should deal with the runtime variability in an automated way, so we do not require human intervention at runtime. %\jesus{I'm sure that automation is a concern, but not if this is the right description}

\item \emph{Assurances}: besides meeting the rules, compliance is also about proving that the system effectively complies.

\item \emph{Performance}: as usual at runtime, the system should be able to detect compliance issues and respond to them in a reasonably efficient way.
\end{itemize}
%\jesus{Complete this paragraph}

%% Variability
%% Automation
%% Assurance
%% Performance







%\jesus{connect the related work with the rest of the section}
%Compliance at runtime issues have been already considered in the literature. \citet{birukou2010integrated} propose a runtime compliance governance approach for Service Oriented Architectures, from modelling of compliance requirements to runtime monitoring of the current compliance state.
%\citet{ly2015compliance} and \citet{barnawi2015runtime} specifically focus on the runtime monitoring of business processes, proposing a framework to compare the different approaches in the literature \cite{ly2015compliance} and particular techniques for process monitoring in the cloud \cite{barnawi2015runtime}.
%\citet{koetter2013unifying} even talk about adaptation in the compliance management, and propose a configurable compliance descriptors to link compliance requirements with their implementation as controls on the system.
%\citet{boella2013managing} are concerned about the impact of changes in the system and regulations, and their impact on the compliance level. Although all these works highlight particular issues on runtime compliance, they adhere to such specific issues. On the contrary, in this paper we try to envision a comprehensive approach to deal with runtime variability in compliance.

%The changes in the operating environment occur much faster and oftener than in the system or the compliance sources. 
%For example, in the \paas scenario, new clients may appear and request the platform with different compliance needs, whose controls could conflict with existing clients.
%In the \byod scenario, new devices may appear at runtime, or the configuration or apps of the existing ones may change, which could potentially diminish the compliance level.
%Consequently, we need an approach to deal with this runtime variability in compliance, which should complement the existing traditional compliance approaches.

%\jesus{bring this to the problem section}
%As far as we are aware, most of the research on compliance regards the system, the compliance sources and the different stages and outputs of the compliance lifecycle. 
%However, the impact of the runtime variability has no received the required attention from the literature. Following, we describe two scenarios where this variability and its impact on compliance is evident.
%\jesus{I may need an example of how the runtime variability in the operating environments affects compliance.}



%The previously described scenarios also introduce the \emph{operating environment} as an extra element that affects compliance. We consider the operating environment as everything that affects the system and the compliance sources that apply, but it is not under direct control of the system. For instance, in the \paas scenario, the platform users, their compliance needs and the platform containers under their control are the operating environment.  
%In the case of the \byod scenario, the hospital employers and their devices make up the operating environment.

%\jesus{examples of particular changes/runtime variability that affect compliance}




%\jesus{intro and compliance scope of this paper}
%Although compliance involves organisations, companies, systems and more actors, in this paper we focus on and take the point of view of IT systems and their implementation of compliance. 
%In this section, we describe the particular compliance problem we address and its context. First, present an overview of compliance for IT systems, setting forth the main vocabulary and concepts. Second, we describe two particular scenarios, related to the cloud and \byod, where runtime variability affects compliance. Finally, we discuss in general terms the impact of runtime variability on compliance.



%\subsection{Compliance Overview}
%
%%\jesus{compliance introduction and meaning. compliance in SE. main elements (sources and system)}
%
%
%\subsection{Motivating Scenarios}
%
%In this section, we describe two highly dynamic and distributed scenarios, which poses additional challenges for compliance. In the first one, we present a \paas that has to respond to the compliance needs of different clients, while the second one is about a company implementing \byod while complying with \hipaa. Both scenarios help us motivate the problem of runtime variability in compliance, and the need of adaptive compliance as a solution.
%
%\subsubsection{PaaS Scenario}
%
%
%\subsubsection{BYOD Scenario}
%
%%\byod policies present multiple benefits but at the same time leads to new challenges, especially in security and privacy terms. 
%\byod refers to the employer policy of permitting employees to bring and use their personally owned devices (e.g. smartphones, laptop, tablets...) to access company resources. On the one hand, this practice is related to a productivity increase by the employees, while reducing required employer investment on employees equipment. On the other hand, \byod leads to serious privacy and security issues~\cite{miller2012byod}. 
%%% I have to reduce the second part of this paragraph
%From the employer's side, security is the main concern: the network could be infected because of malware from those devices (often untrusted), or sensitive data may end in user's devices, losing control of it. Before \byod, the devices were totally managed by the employer, which most the time ensured compliant by design. From the employee's side, however, the main issue is privacy: employers might want to have some degree of control or monitoring on employee's devices, which are also used for personal purposes. In this sense, the line between personal and employer data is blurred.
%
%\begin{figure}
%\includegraphics[scale=0.45]{figures/BYODScenario.pdf} 
%\caption{BYOD Scenario}
%\label{fig:BYODScenario}
%\end{figure}
%
%%% BYOD particular scenario
%In our particular \byod scenario, we present a hospital in the US that allows their employees to use their own devices. At the same time, the hospital is forced to comply with the \hipaa, and they are also willing to comply with the ISO standard on privacy (ISO/IEC 29100) \cite{iso29100}. 
%Due to \byod, many doctors in this hospital employ their own devices to check and register patient health's conditions. For example, Doctor1 employs his own iPad, while Doctor2 uses his Android tablet for this purpose (Figure~\ref{fig:BYODScenario}). The doctors employ these devices also for personal use, as usual in \byod, so they have installed different apps and have personal files in the devices. While the device of Doctor1 seems secure, the Doctor2's tablet allows to install apps from unknown sources and does not have an antivirus.
%
%Existing issues and threats of \byod get magnified when, for example, a hospital has to comply with \hipaa. 
%A stolen, lost or even compromised device may lead to protected health information leaks, and consequently to settlements and fines, something that has already happened \footnote{http://www.healthcarefinancenews.com/news/lahey-pays-850k-widespread-hipaa-non-compliance}. This means that if our doctors lose their personal devices, or get them infected by malware (likely to happen for Doctor2), the hospital might violate \hipaa compliance.
%Besides, the variability of devices and their configuration and installed apps in \byod pose an additional challenge for compliance. For example, our two doctors have two different devices (iPad and Android tablet), each one with different configuration, apps and their own threats, as shown in Figure~\ref{fig:BYODScenario}. 
%Although there are technologies to manage the connected devices (e.g, Mobile Device Management) remotely to configure them in the proper way for compliance, this might go against the privacy of the users. For example, analysing the outgoing traffic of the doctors devices to ensure compliance may invade their privacy.




%% particular policies
%% - support for blackberry, iOS and Android. particular configurations will be neccesary
%% - require the installation of a company app
%% - require the installation of particular antivirus
%% - devices should not be rooted or jailbroken
%% - devices should be updated to the newest available OS version
%% - healthcare data can only be accessed using containerization technology.

%% resources:
%% - internal network
%% - virtual machines & servers
%% - shared storage
%% - DB

%% technologies:
%% - Mobile-device Management (MDM) + NAC (Network Access Control)
%% - Containerization

%% issues and questions:
%% - maybe am I doing something that is already done?
%%   + the enabling technology already exists. 
%%   + which are the research challenges then?
%%   + RESEARCH CHALLENGE: How to be compliant with regulations and standards while allowing BYOD?
%% - where are the jurisdictions in this scenario? 
%%   + It could be the OS or type of device (Android, iOS, Windows...)
%% - what's the differente between adaptive security and adaptive compliance?
%%   + ??




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> relatedWork.tex <==
\section{Related Work}
\label{sec:related}

Compliance has attracted much attention from software engineering academics, especially in the areas of requirements engineering, \soa, cloud computing and \bpm. This has led several authors to survey the state of the art for general or particular purposes.
Most of the works in requirements engineering, as \citet{otto2007addressing} show, focus on interpreting the compliance sources and extracting, representing, analysing and reconciling compliance requirements. 
In the cloud area, \citet{martens2011risk} propose a reference model for risk and compliance management, based on a systematic literature review. However, the most prolific area for compliance is \bpm. In this sense, Tilburg University \cite{Tilburg08} present a literature review, in the context of an European project, focused on the discovery, specification and improvement aspects of compliance for services and business processes. \citet{fellman2014state} also survey the general state of the art cataloguing the literature in different dimensions, while \citet{el2012business} analyses the solutions proposed on regulatory compliance management. In this work we survey the literature in all these areas, but in our case to find out how good adaptive compliance can be supported with the existing research.

Compliance at runtime issues have been already considered in the literature. \citet{birukou2010integrated} propose a runtime compliance governance approach for Service Oriented Architectures, from modelling of compliance requirements to runtime monitoring of the current compliance state.
\citet{ly2015compliance} and \citet{barnawi2015runtime} specifically focus on the runtime monitoring of business processes, proposing a framework to compare the different approaches in the literature \cite{ly2015compliance} and particular techniques for process monitoring in the cloud \cite{barnawi2015runtime}.
\citet{koetter2013unifying} even talk about adaptation in the compliance management, and propose a configurable compliance descriptors to link compliance requirements with their implementation as controls on the system.
\citet{boella2013managing} are concerned about the impact of changes in the system and regulations, and their impact on the compliance level. Although all these works highlight particular issues on runtime compliance, they adhere to such specific issues. On the contrary, in this paper we try to envision a comprehensive approach to deal with runtime variability in compliance.

%% compliance governance and comprehensive approaches
Some other authors have proposed comprehensive compliance approaches to assist the compliance process during its whole lifecycle, especially for business processes. \citet{el2008towards} and \citet{ly2012enabling} discuss the requirements and challenges of frameworks for business process compliance management, and present their own approaches in this sense. In a similar line, \citet{cabanillas2011exploring} propose the concept of business process compliance management system, together with a lifecycle for compliance management and a set of challenges. \citet{ramezani2012separating} advocate for the separation of the compliance management from the business process, and also propose a lifecycle in this sense. \citet{tran2012compliance} propose a model-driven approach for compliance management in process-based SOA environments, with multiple views addressing different compliance concerns. \citet{daniel2009business} present a governance approach for SOA-based business processes, covering the whole lifecycle.



\jesus{should we include here and compare the compliance lifecycle proposals? We can discuss them here or in the compliance overview.}
%% lifecycle approaches:
%% - \citet{cabanillas2011exploring}
%% - \citet{ramezani2012separating}
%% - \citet{daniel2009business}
%% - \cite{Tilburg08}
%% - \citet{fellman2014state} %% for compliance checking



